Self-Organizing Interaction Spaces: A Framework for Engineering Pervasive Applications in Mobile and Distributed Environments

The rapid adoption of pervasive and mobile computing has led to an unprecedented rate of data production and consumption by mobile applications at the network edge. These applications often require interactions such as data exchange, behavior coordination, and collaboration, which are typically mediated by cloud servers. While cloud computing has been effective for distributed systems, challenges like latency, cost, and intermittent connectivity persist. With the advent of 5G technology, features like location-awareness and device-to-device (D2D) communication enable a more distributed and adaptive architecture. This paper introduces Self-Organizing Interaction Spaces (SOIS), a novel framework for engineering pervasive applications. SOIS leverages the dynamic and heterogeneous nature of mobile nodes, allowing them to form adaptive organizational structures based on their individual and social contexts. The framework provides two key abstractions for modeling and programming pervasive applications using an organizational mindset and mechanisms for adapting dynamic organizational structures. Case examples and performance evaluations of a simulated mobile crowd-sensing application demonstrate the feasibility and benefits of SOIS. Results highlight its potential to enhance efficiency and reduce reliance on traditional cloud models, paving the way for innovative solutions in mobile and distributed environments.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/mobile_multiplayer_game.tex <==
\subsection{Mobile Multiplayer Game}

The next ultimate gaming experience may follow the fusion of the physical and virtual worlds, where the dimensions and assets of our physical reality are augmented with elements from the virtual reality. This combination would allow users to go beyond the limitations of their homes and enjoy the outside and the physical company of other people while still been able to employ the power of their digital equipments to extend their perception of the world with rich elements and narratives provided by the game industry. To achieve this, interactions must have a low latency and last as long as possible, meaning an efficient use of devices battery.

The potential improvements to wireless communications proposed by 5G include a device-2-device communication that would allow devices within a given zone to communicate with high throughputs. In a real-time mobile multiplayer game (MMG), such feature would allow the formation of interaction spaces in which devices would be able to synchronize and update the game state with low latency. However, in a pure P2P game architecture, some players may use modified applications to have advantage over other players (cheating). This is one the main reasons for the use of authoritative servers~\cite{}, which are generally deployed in the cloud -- adding network latency that may not fit with real-time constraints. To address this issue, we propose a P2P architecture with peer review of the game state update. In this model, each update to the game state performed by a node is checked by a peer node dynamically chosen. Thus, if a node updates the game to an invalid state, there is a great chance such violation would be detected. Figures~\ref{fig:} and~\ref{fig:} illustrate a classic client-server architecture and the aforementioned P2P architecture.

FIGURE: a) classic client-server architecture; b) our proposed P2P architecture

The P2P with peer review architecture implies the dynamic selection of a \textit{reviewer} for each of the available node. For obvious reasons, a single node should not accumulate this role, i.e., reviewers should be evenly distributed among nodes. A simple scheme would be to randomly allocate this role to one of the nodes which have not yet been chosen. While the details of this approach are out of the scope of this paper, it illustrates how a data-intensive and delay-sensitive application could explore the potential of a self-organizing edge space. In the next section, we describe the abstractions and the self-organization mechanisms for the engineering and execution of interactive mobile applications.

%While this solution would still rely on backend servers for processing and persisting game data, a pure cloud-based solution would imply a significant amount of data to be transfered back and forward, increasing latency and the use of mobile data plans. In addition to the election and replication of roles, the physical-virtual space mapping tends to be more coarse and fuzzy than previous example. For instance, a game may choose city parks as arena for users interaction. Accordingly, a \textit{game session group} could have the geolocation coordinates of a park region as its membership criteria. Once devices are within the same session group and a server role is elected, the game session may start.


%To achieve a fair use of resources, the server role should be rotated among existing group members even before the active role have quit the system. 

%To prevent battery drain, a GPS role can be assigned to fewer members and broadcasted using low energy bluetooth.

==> sections/plots.tex <==
%Draw graphics
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\pgfplotsset{compat=newest}
\pgfplotscreateplotcyclelist{my chart colors}{%
blue, solid, every mark/.append style={solid, fill=blue}, mark=*\\%
red, solid, every mark/.append style={solid, fill=red}, mark=square*\\%
brown, solid, every mark/.append style={solid, fill=brown}, mark=triangle*\\%
cyan, solid, every mark/.append style={solid, fill=gray}, mark=diamond*\\%
black, dashdotted, every mark/.append style={solid, fill=red}, mark=halfdiamond*\\%
olive, dashdotted, every mark/.append style={solid, fill=green}, mark=halfcircle*\\%
orange, dashdotted, every mark/.append style={solid, fill=gray}, mark=*\\%
purple, dashdotted, every mark/.append style={solid, fill=blue}, mark=halfsquare left*\\%
teal, densely dashed, every mark/.append style={solid, fill=green}, mark=oplus*\\%
violet, densely dashed, every mark/.append style={solid, fill=gray}, mark=diamond*\\%
magenta, densely dashed, every mark/.append style={solid, fill=blue}, mark=triangle*\\%
lime, densely dashed, every mark/.append style={solid, fill=red}, mark=square*\\%
}

\newcommand{\errorband}[5][]{ % x column, y column, error column, optional argument for setting style of the area plot
\pgfplotstableread[col sep=comma, skip first n=2]{#2}\datatable
    % Lower bound (invisible plot)
    \addplot [draw=none, stack plots=y, forget plot] table [
        x={#3},
        y expr=\thisrow{#4}-\thisrow{#5}
    ] {\datatable};

    % Stack twice the error, draw as area plot
    \addplot [draw=none, fill=gray!40, stack plots=y, area legend, #1] table [
        x={#3},
        y expr=2*\thisrow{#5}
    ] {\datatable} \closedcycle;

    % Reset stack using invisible plot
    \addplot [forget plot, stack plots=y,draw=none] table [x={#3}, y expr=-(\thisrow{#4}+\thisrow{#5})] {\datatable};
}

==> sections/self_adaptation.tex <==
\section{Self-adaptation}\label{sec:self_adaptation}

\subsection{Role Cardinality} 

The relation between the number of instances of a given role and different non-functional attributes of a system may be straightforward (e.g., the number of similar sensors in a cluster and the accuracy of the information this cluster provides) or less evident (e.g., the number of replicas of a component and the availability or reliability of the functionality it provides). In addition, considering the scenario of mobile applications, the mapping between role cardinality and these attributes tend to change according to the context they operate, i.e., it may depend on which devices are assigned to the role (e.g., more/less powerful computational resources, more/less accurate sensors) and the state of each device (e.g., more/less battery, more/less signal strength). Hence, in order to avoid violations of these attributes, the cardinality of a role must reflect the circumstances. %To this end, we propose a last, but not least important mechanism for adapting the application organization. 

\subsection{Group Cardinality} 

Since the encounter of mobile application nodes is opportunistic and not deterministic, group membership criteria specifies no size threshold or limit: as long as a node satisfies the group's membership criteria, it becomes/remains a member. This choice avoids the need for a group membership control by a trustful component and simplifies the grouping process. Accordingly, the size of a group, kept stable the membership criteria satisfaction by each of its members, can only be changed by making this criteria more relaxed or strict. 

Whereas the self-organization mechanisms presented address the \textit{solution space}, i.e., which nodes provide which application functionality, here the \textit{requirement space} is the target of the adaptation, i.e., the application requirements evolve to accommodate situations in which no solution can satisfy those requirements~\cite{RELAX}. 

